A Survey of Code-switched Arabic NLP: Progress, Challenges, and Future Directions

Language in the Arab world presents a complex diglossic and multilingual setting, involving the use of Modern Standard Arabic, various dialects and sub-dialects, as well as multiple European languages. This diverse linguistic landscape has given rise to code-switching, both within Arabic varieties and between Arabic and foreign languages. The widespread occurrence of code-switching across the region makes it vital to address these linguistic needs when developing language technologies. In this paper, we provide a review of the current literature in the field of code-switched Arabic NLP, offering a broad perspective on ongoing efforts, challenges, research gaps, and recommendations for future research directions.

==> commented_text <==
%This evolution highlights the dynamic nature of language contact and the ongoing interplay between linguistic identity and historical forces.

%The history of code-switching in the Arab world is deeply rooted in significant historical events.  

%Throughout history, languages have been mixed and intertwined, affecting each other on a continuum where words on one end, are borrowed, with or without receiving morphological or phonological modifications and become integrated into a language , and on another end, multiple languages are used in conjunction, producing CSW. Given the Islamic conquests later followed by European colonizations in Arab countries, code-switching can be found between many languages, such as Persian-Arabic \cite{}, .., . 

%In the dynamic landscape of language, code-switching (CSW) has emerged as a fascinating linguistic phenomenon where individuals effortlessly alternate between multiple languages within the same discourse. Historically, languages have continually mixed and influenced each other. This mixing results in a continuum where, on one end, words are borrowed and integrated with or without morphological or phonological changes, and on the other end, multiple languages are used concurrently, leading to CSW. 

%Arabic is a classical example of a diglossic language \citep{Fer59}. There are three types of Arabic: classical Arabic, Modern Standard Arabic (MSA), and Dialectal Arabic (DA). The classical Arabic is the most formal type of Arabic, which is used in the Quran and early Islamic literature. MSA is a direct descendant of the classical Arabic and is the official form of Arabic taught in schools. MSA is used in formal contexts such as formal writings and speeches, news broadcasts, movies' subtitling and education, however, it is not used in everyday conversations. MSA is considered as a second language for all Arabic speakers and serves as a lingua franca across the Arab countries. Dialectal Arabic is the language used in everyday conversations as well as informal writings such as blogs, chats and comments on on-line social media. Besides the three forms of Arabic, code-switching is present across different variants of Arabic (MSA and dialectal) as well across Arabic and foreign languages, mostly English and French. The complexity of code-switching is then further compounded by challenges posed by dialectal Arabic, including is a low-resourcefulness, morphologically richness and orthographic unstandardization \citep{habash2012conventional,habash2012morphological}. In the case of Arabic-foreign code-switching, challenges are also introduced as the secondary language is a non-semitic language, where both languages have different scripts.

%, as shown in Figure \ref{fig:colonization}, 
% the Middle East has seen a spread of European colonialism across its countries
%Several Arab countries have a long history of colonization, 
%where the French, British and Italian colonies competed against each other, securing their own national identities as well as their interest in the region \cite{Mil18}
